Spectral asymptotics for large skew-symmetric perturbations of the harmonic oscillator

Originally motivated by a stability problem in Fluid Mechanics, we study the spectral and pseudospectral properties of the differential operator $H_\epsilon = -\partial_x^2 + x^2 + i\epsilon^{-1}f(x)$ on $L^2(R)$, where $f$ is a real-valued function and $\epsilon > 0$ a small parameter. We define $\Sigma(\epsilon)$ as the infimum of the real part of the spectrum of $H_\epsilon$, and $\Psi(\epsilon)^{-1}$ as the supremum of the norm of the resolvent of $H_\epsilon$ along the imaginary axis. Under appropriate conditions on $f$, we show that both quantities $\Sigma(\epsilon)$, $\Psi(\epsilon)$ go to infinity as $\epsilon \to 0$, and we give precise estimates of the growth rate of $\Psi(\epsilon)$. We also provide an example where $\Sigma(\epsilon)$ is much larger than $\Psi(\epsilon)$ if $\epsilon$ is small. Our main results are established using variational "hypocoercive" methods, localization techniques and semiclassical subelliptic estimates.

==> Fig1.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       7.90       0.40 {$|x|$}
\point      -0.10       4.50 {$\beta(x)$}
\point      -2.00       3.90 {$\beta_0\,\epsilon^{-\frac{k}{k+4}}$}
\point      -1.20       1.00 {$\beta_0$}
\point       2.20      -0.40 {$A$}
\point       4.90      -0.40 {$B_\epsilon$}
}}


==> Fig3.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       8.40       0.50 {$\lambda$}
\point       0.10       6.80 {$\kappa(\epsilon,\lambda)$}
\point      -1.80       6.00 {$\OO(\epsilon^{\frac{2}{k+4}})$}
\point      -1.70       4.70 {$\OO(\epsilon^{1/2})$}
\point      -1.70       3.90 {$\OO(\epsilon^{1/2})$}
\point      -1.80       2.90 {$\OO(\epsilon^{\frac{2}{k+2}})$}
\point      -1.70       1.20 {$\OO(\epsilon^{2/3})$}
\point      -1.40       0.40 {$\OO(\epsilon)$}
\point       0.85      -0.20 {$0$}
\point       1.10       0.50 {$\leftarrow \OO(\epsilon^{-\frac{4}{k+4}})$}
\point       4.10      -0.20 {$c_1\,\epsilon^{-1}$}
\point       6.60      -0.20 {$c_2\,\epsilon^{-1}$}
}}

==> Fig4.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point      -1.50       3.30 {\begin{sideways}
$\log(\Sigma(\epsilon))$\end{sideways}}
\point       3.00      -0.20 {$\log(\epsilon)$}
\point      -0.20       6.60 {$k=1$}
\point      -0.20       5.50 {$k=2$}
\point      -0.20       3.40 {$k=4$}
}}

